ReDirTrans: Latent-to-Latent Translation for Gaze and Head Redirection

Learning-based gaze estimation methods require large amounts of training data with accurate gaze annotations. Facing such demanding requirements of gaze data collection and annotation, several image synthesis methods were proposed, which successfully redirected gaze directions precisely given the assigned conditions. However, these methods focused on changing gaze directions of the images that only include eyes or restricted ranges of faces with low resolution (less than $128\times128$) to largely reduce interference from other attributes such as hairs, which limits application scenarios. To cope with this limitation, we proposed a portable network, called ReDirTrans, achieving latent-to-latent translation for redirecting gaze directions and head orientations in an interpretable manner. ReDirTrans projects input latent vectors into aimed-attribute embeddings only and redirects these embeddings with assigned pitch and yaw values. Then both the initial and edited embeddings are projected back (deprojected) to the initial latent space as residuals to modify the input latent vectors by subtraction and addition, representing old status removal and new status addition. The projection of aimed attributes only and subtraction-addition operations for status replacement essentially mitigate impacts on other attributes and the distribution of latent vectors. Thus, by combining ReDirTrans with a pretrained fixed e4e-StyleGAN pair, we created ReDirTrans-GAN, which enables accurately redirecting gaze in full-face images with $1024\times1024$ resolution while preserving other attributes such as identity, expression, and hairstyle. Furthermore, we presented improvements for the downstream learning-based gaze estimation task, using redirected samples as dataset augmentation.

==> 1-figures/fig_redir_w_targets.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.249\linewidth}
        \begin{minipage}[b]{1\linewidth}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00009-hp_0.43_-0.02-g_-0.14_0.02-raw-src.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00021-hp_-0.10_0.03-g_-0.07_-0.13-raw-src.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00088-hp_0.27_-0.16-g_-0.01_-0.12-raw-src.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00104-hp_0.10_-0.01-g_-0.27_0.13-raw-src.jpg}
        \end{minipage}
    \caption{Input}
    \label{fig:input4}
  \end{subfigure}
  \hspace{-0.015\linewidth}
  \centering
    \begin{subfigure}{0.249\linewidth}
        \begin{minipage}[b]{1\linewidth}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00009-hp_0.43_-0.02-g_-0.14_0.02-raw.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00021-hp_-0.10_0.03-g_-0.07_-0.13-raw.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00088-hp_0.27_-0.16-g_-0.01_-0.12-raw.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00104-hp_0.10_-0.01-g_-0.27_0.13-raw.jpg}
        \end{minipage}
    \caption{e4e Inversion}
    \label{fig:e4e_inv3}
  \end{subfigure}
  \hspace{-0.021\linewidth}
  \centering
    \begin{subfigure}{0.249\linewidth}
        \begin{minipage}[b]{1\linewidth}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00009-hp_0.43_-0.02-g_-0.14_0.02.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00021-hp_-0.10_0.03-g_-0.07_-0.13.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00088-hp_0.27_-0.16-g_-0.01_-0.12.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00104-hp_0.10_-0.01-g_-0.27_0.13.jpg}
        \end{minipage}
    \caption{Redirection}
    \label{fig:redirection}
  \end{subfigure}
  \hspace{-0.021\linewidth}
  \centering
    \begin{subfigure}{0.249\linewidth}
        \begin{minipage}[b]{1\linewidth}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00009-hp_0.43_-0.02-g_-0.14_0.02-tar.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00021-hp_-0.10_0.03-g_-0.07_-0.13-tar.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00088-hp_0.27_-0.16-g_-0.01_-0.12-tar.jpg}
        \includegraphics[width=1\linewidth]{figs/redir_w_tar/00104-hp_0.10_-0.01-g_-0.27_0.13-tar.jpg}
        \end{minipage}
    \caption{Target}
    \label{fig:target}
  \end{subfigure}
  \caption{Redirection results of the GazeCapture test subset with target images from the same person. Col. c includes the redirection results on the basis of inverted results in Col. b with the attributes' conditions provided by target images from Col. d. The gaze directions' differences between input (Col. a) and inverted results (Col. b) cause inconsistent redirection process.}
  \label{fig_w_target}
\end{figure}

==> _constants.tex <==
\def\cvprPaperID{7405}
\def\confName{CVPR}
\def\confYear{2023}

\def\paperTitle{ReDirTrans: Latent-to-Latent Translation for Gaze and Head Redirection}

\def\authorBlock{
    Shiwei Jin $^{1}$,  
    Zhen Wang $^{2}$, 
    Lei Wang $^{2}$, 
    Ning Bi $^{2}$, 
    Truong Nguyen $^{1}$ \\
    $^{1}$ ECE Dept. UC San Diego, $^{2}$ Qualcomm Technologies, Inc. \\
    {\tt\small \{sjin, tqn001\}@eng.ucsd.edu, \{zhewang, wlei, nbi\}@qti.qualcomm.com}
}

% Compilation vars
\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> _macros.tex <==
%% PACKAGES (also see cvpr_header.tex)

\usepackage{times}
\usepackage{microtype}
\usepackage{epsfig}
\usepackage[table,xcdraw]{xcolor}
\usepackage{caption}
\usepackage{float}
\usepackage{placeins}
\usepackage{color, colortbl}
\usepackage{stfloats}
\usepackage[inline, shortlabels]{enumitem}
\usepackage{tabularx}
\usepackage{xstring}
\usepackage{multirow}
\usepackage{xspace}
\usepackage{url}
\usepackage{subcaption}
\usepackage{xcolor}
\usepackage{svg}
\usepackage[hang,flushmargin]{footmisc}
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

% Unfortunately, this package interferes with arxiv's stamp
\ifcamera \usepackage[accsupp]{axessibility} \fi

%% MACROS

% \newcommand{\authorname}[1]{{\textcolor{blue}{[Author: #1]}}}
% ...

% \newcommand{\commandname}{string\xspace}
% \definecolor{colorname}{rgb}{0.92,0.49,0.19}

% General

\newcommand{\nbf}[1]{{\noindent \textbf{#1.}}}

\newcommand{\supp}{supplemental material\xspace}
\ifarxiv \renewcommand{\supp}{appendix\xspace} \fi

\newcommand{\todo}[1]{{\textcolor{red}{[TODO: #1]}}}

% Reviewer commands (1 to 5), e.g. \R{1}, \R{2}
\newcommand{\R}[1]{{%
    \textbf{%
        \ifstrequal{#1}{1}{\textcolor{red}{R#1}}{%
        \ifstrequal{#1}{2}{\textcolor{teal}{R#1}}{%
        \ifstrequal{#1}{3}{\textcolor{blue}{R#1}}{%
        \ifstrequal{#1}{4}{\textcolor{teal}{R#1}}{%
                           \textcolor{cyan}{R#1}%
        }}}}%
    }%
}}

\newcommand*\circled[1]{\tikz[baseline=(char.base)]{% 
\node[shape=circle,fill=yellow,draw,inner sep=1pt] (char) {#1};}}

\newenvironment{packed_enum}{
\begin{enumerate}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}

\newenvironment{packed_item}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{2pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}



==> cvpr_header.tex <==
\ifreview \usepackage[review]{cvpr} \fi
\ifarxiv \usepackage[pagenumbers]{cvpr} \fi
\ifrebuttal \usepackage[rebuttal]{cvpr} \fi
\ifcamera \usepackage{cvpr} \fi

\usepackage{graphicx}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{booktabs}

\usepackage{tikz}

\input{_macros}  % Add packages to _macros.tex

%% For cross-referencing labels between documents
\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}
%%

\usepackage[pagebackref,breaklinks,colorlinks]{hyperref}
\usepackage[capitalize]{cleveref}
\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\frenchspacing


==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}

